Adaptive Data-Driven Prediction in a Building Control Hierarchy: A Case Study of Demand Response in Switzerland

By providing various services, such as Demand Response (DR), buildings can play a crucial role in the energy market due to their significant energy consumption. However, effectively commissioning buildings for such desired functionalities requires significant expert knowledge and design effort, considering the variations in building dynamics and intended use. In this study, we introduce an adaptive data-driven prediction scheme based on Willems' Fundamental Lemma within the building control hierarchy. This scheme offers a versatile, flexible, and user-friendly interface for diverse prediction and control objectives. We provide an easy-to-use tuning process and an adaptive update pipeline for the scheme, both validated through extensive prediction tests. We evaluate the proposed scheme by coordinating a building and an energy storage system to provide Secondary Frequency Control (SFC) in a Swiss DR program. Specifically, we integrate the scheme into a three-layer hierarchical SFC control framework, and each layer of this hierarchy is designed to achieve distinct operational goals. Apart from its flexibility, our approach significantly improves cost efficiency, resulting in a 28.74% reduction in operating costs compared to a conventional control scheme, as demonstrated by a 52-day experiment in an actual building. Our findings emphasize the potential of the proposed scheme to reduce the commissioning costs of advanced building control strategies and to facilitate the adoption of new techniques in building control.

==> figs/deleted.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2. detrend, split,

\subsubsection{Detrending} Prepocessing the data by removing a trend helps to remove some kind of distortion in regression. Here the trend is defined as the average value of the historical data involved in the Hankel matrix:
\begin{align*}
    u_{trend} =  \sum \frac{u_d^{M}}{M}, \; 
    w_{trend} =  \sum \frac{w_d^{M}}{M}, \; 
    y_{trend} =  \sum \frac{y_d^{M}}{M},
\end{align*}
Then the prediction \eqref{eqn:deepc_pred2} becomes:
\begin{subequations}\label{eqn:deepc_pred3}
\begin{align}
        &\;\mathbf{y}_{pred} = \Han_{L,pred}(y_\textbf{d}-y_{trend})g + y_{trend}\;, \label{eqn:deepc_pred3_y} \\ 
        & \;\begin{bmatrix}
        g\\\kappa
        \end{bmatrix} = G_{detrend}^{-1}\begin{bmatrix}\Han_{L,init}(y_\textbf{d}^M-y_{trend})^\top \mathbf{y}_{init}-y_{trend}\\
        \mathbf{u}_{init}-u_{trend}\\
        \mathbf{w}_{init}-w_{trend}\\
        \mathbf{u}_{pred}-u_{trend}\\
        \mathbf{w}_{pred}-w_{trend}\end{bmatrix}\;,
\end{align}
\end{subequations}
where $G_{detrend}$ is computed similar to~\eqref{eqn:deepc_pred2_sub3} by the detrended Hankel matrices.


From the aspect of dynamics, the trends relates to the steady state of the building dynamics. Heuristicly, detrended data capture the linearized dynamics around the operation point so that DeePC's performance is improved.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tuning section: 12 and 96
We start with a short-term prediction analysis, by choosing $N_pred=12$, which means 3 hours with a 15-minute sampling period.
Then a series of techniques are elaborated to increase the prediction ability. In the end, the results by the same tests for $N_{}=96$ (24 hours) will be summarized. The best prediction way will be used in \textbf{Predictive building controller} ($N_{}=12$) and \textbf{Day-ahead planner} ($N_{}=96$).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AGC prediction
By utilizing historical data spanning 200 days in 2019, a Gaussian model is learned to predict the AGC sequence at 15-minute intervals. The accuracy of the AGC predictions is evaluated using root-mean-square error (RMSE) analysis on the validation dataset (150-day AGC signals in 2019). Figure~\ref{fig:pdf_agc_rmse} displays the results of the RMSE analysis and the Gaussian model outperforms the persistence method. To ensure safe AGC tracking, a conservative bound of $|e_a| \leq 0.2$ is chosen. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/pdf_agc_rmse.pdf}
    \caption{RMSE of the AGC prediction error. Compare the prediction by the Gaussian model and persistence method.}
    \label{fig:pdf_agc_rmse}
\end{figure}

==> figs/figure_agc_prediction.tex <==
 \definecolor{myblue}{rgb}{0.20, 0.6, 0.78}
\definecolor{mygreen}{rgb}{0.2,0.8,0.2}
\definecolor{myred}{rgb}{0.5,0,0}

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    date coordinates in=x,
    % date ZERO=2021-05-13 00:00,   % <-- needs to be set for v1.12 and below
    xmin=2021-05-13 23:59,
    xmax=2021-05-14 24:00,
    % set `xtick distance' to 3 hours (3/24)
    xtick distance=0.125,
    % set the label style of the `xtick's
    % xticklabel=\year.\month.\day\ \hour:\minute]
    xticklabel=\hour:\minute,
    % xmin=1, xmax=102,
    ymin=5, ymax= 30.5,
    enlargelimits=false,
    clip=true,
    grid=major,
    mark size=0.5pt,
    width=0.9\linewidth,
    height=0.6\linewidth,
    ylabel = {$y$ (indoor temperature [$^{\circ} C$])},
    xlabel= time,
    ylabel style={at={(axis description cs:0.05,0.5)}},
    xlabel style={at={(axis description cs:0.5,0.05)}},
    legend columns=3,
    label style={font=\scriptsize},
    ticklabel style = {font=\scriptsize},
    legend style={
    	font=\footnotesize,
    	draw=none,
		at={(0.5,1.03)},
        anchor=south
    }    
    ]
    
    \pgfplotstableread[col sep=comma]{data/polydome_min.dat}{\dat}

    \addplot+ [ultra thick,smooth, mark=*, mark options={fill=white, scale=1,line width = 0.1pt},myred] table [x={tt}, y={y}] {\dat};    
    \addlegendentry{Output: y}
    
    \addlegendimage{line legend,ultra thick,smooth, mark=*, mark options={fill=white, scale=1,line width = 0.2pt}, myblue}
    \addlegendentry{\change{Input}: u}       
    
    \addplot+ [thick,brown,dashed,mark = none] table [x={tt}, y={max}] {\dat};
    \addplot+ [thick,brown, dashed, mark = none] table [x={tt}, y={min}] {\dat};
    \addlegendentry{Constraint}     
    
    \end{axis}
     
    
    \end{tikzpicture}
    \caption{RMSE of the AGC prediction error with respect to prediction time. }
    \label{fig:exp_polydome_2}     
 \end{figure}
